Category-Level Articulated Object Pose Estimation

This project addresses the task of category-level pose estimation for articulated objects from a single depth image. We present a novel category-level approach that correctly accommodates object instances previously unseen during training. We introduce Articulation-aware Normalized Coordinate Space Hierarchy (ANCSH) - a canonical representation for different articulated objects in a given category. As the key to achieve intra-category generalization, the representation constructs a canonical object space as well as a set of canonical part spaces. The canonical object space normalizes the object orientation,scales and articulations (e.g. joint parameters and states) while each canonical part space further normalizes its part pose and scale. We develop a deep network based on PointNet++ that predicts ANCSH from a single depth point cloud, including part segmentation, normalized coordinates, and joint parameters in the canonical object space. By leveraging the canonicalized joints, we demonstrate: 1) improved performance in part pose and scale estimations using the induced kinematic constraints from joints; 2) high accuracy for joint parameter estimation in camera space.

==> tex/app.tex <==
\section{Implementation Details}
% \todo{@Xiaolong}
We use Tensorflow 1.10 to build our models and run the experiments for all categories. The input is uniformly sampled points from the whole back-projected depth point cloud, with points number $N$ set to 1024.  We train our model on a single Nvidia V100 GPU with batch size of 16 across the experiments. The initial learning rate is set to 0.001, with a decay factor of 0.7 every 200k steps. From the observations of our experiments, the loss will usually converge well after $>150k$ steps in less than one day. 

\section{Data generation and statistics} 
We render synthetic depth images using the object 3D model provided in the Shape2Motion dataset \cite{wang2019shape2motion} and SAPIEN dataset \cite{xiang2020sapien}. Both datasets provide the descriptions of the object geometry and articulation information, which we leverage for generating ground truths. 
During rendering, the program automatically generates random joint states for each object instance, according to its joint motion ranges.  Then the depth images and corresponding ground truth masks are rendered from a set of random camera viewpoints. We also filter out camera poses where some parts of the object are completely  occluded. 
% On average, 30,000 training images for 40 different object instances are generated for each object category.
Figure \ref{fig:part} shows the index definitions of parts for each object category used in the main paper, together with number of object instances splitted for training and testing. 

We use real data from ICCV2015 Articulated Object Challenge \cite{michel2015pose}, which contains RGB-D data with 4 articulated objects: laptop, cabinet, cupboard and toy train. 
 This dataset provides 2 testing sequences for each object. Each sequence contains around 1000 images captured by having a RGB-D camera slowly moving around the object. Objects maintain the same articulation state within each sequence. Each part of the articulated object is annotated with its 6D pose with respect to the known CAD model. Since no training data is provided, we use the provided CAD models to render synthetic depth data, with 10 groups of random articulation status considered.
 %To narrow down the domain gap, 4 sets of articulation parameters are designed to be close to the ones used in the testing stage.
 We render object masks for the testing sequences with Pybullet\cite{coumans2018}. 
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figure/figure5d.pdf}
    % \caption{\textbf{Visualization of part definition}  }
    %https://docs.google.com/drawings/d/1F8NaOgJ1scfSzYHpDyzgvS1L-cFZYJ9dTLXOvAXf4CI/edit?usp=sharing
% \end{figure}
% \begin{table}[h!]
    \centering
    \setlength\tabcolsep{3px}
    \begin{tabular}{c|c|c|c|c|c}
\toprule 
    Category  & \multicolumn{4}{c|}{Part definitions}                    & \multicolumn{1}{c}{Data statistics} \\
\midrule
   & Part 0 & Part 1 & Part 2 & Part 3 & train/test \\
\midrule
\multirow{1}{*}{Eye-} & base   & left & right & - & 39/3\\
glasses &  & temple & temple & & \\
\midrule
Oven &  base   &  door & - & - & 35/3\\
\midrule
\multirow{1}{*}{Washing} & base   &  door & - & - & 42/2 \\
Machine & & & & \\
\midrule
Laptop &  base   &  display & - & - & 78/3\\
\midrule
Drawer &  base   & lowest  & middle & top & 30/2 \\
    \bottomrule
    \end{tabular}
   \caption{\textbf{Synthetic data statistics.} We list part definitions for each object category tested in our experiments on synthetic data, together with the numbers of object instances used for training and testing.  \label{fig:part} }
\vspace{-5mm}
\end{figure}
% \begin{table}[h!]
%     \centering
%     \setlength\tabcolsep{3px}
%     \begin{tabular}{c|c|c|c}
%     \toprule
%   Category  & Methods & angle error & distance error\\
% \midrule

%     \bottomrule
%     \end{tabular}
%     \caption{\textbf{Train/test .}}
%     \label{tab:joint}
% \end{table}

\section{Handling severe occlusion cases}
We carefully examine how ANCSH performs under different levels of occlusion. Compared to our NPCS baseline, our proposed method is still capable of improving the pose estimation under severe occlusion. The occlusion level is defined according to the ratio of visible area with respect to the total mesh surface per part.
\begin{figure}[h]
 \vspace{-2mm}
    \centering
    \includegraphics[width=\linewidth]{figure/figure9s.png}
    \caption{\textbf{ Performance under different occlusion levels.} Data is collected from part 2 of unseen eyeglasses.}
    \label{fig:failures}
    \vspace{-3mm}
    %https://docs.google.com/drawings/d/1F8NaOgJ1scfSzYHpDyzgvS1L-cFZYJ9dTLXOvAXf4CI/edit?usp=sharing
\end{figure}
% \section{Comparison on joints estimation.}
% Table \ref{tab:joint} shows the result comparison on joint parameter estimation for all object categories. The result shows that our approach consistently outperforms the PointNet++ regression baseline on both joint orientation and location accuracy. Note that the prismatic joints in drawers don't have a pivot point so there is no need for evaluating distance error.

% \begin{table}[h!]
%     \centering
%     \setlength\tabcolsep{3px}
%     \begin{tabular}{c|c|c|c}
%     \toprule
%   Category  & Methods & angle error & distance error\\
% \midrule
% \multirow{2}{*}{Eye-} & PointNet++   &  2.9$\degree$, 15.7$\degree$ & 0.129, 0.183\\
%       glasses         &  \nameshort     & \textbf{0.39$\degree$}, \textbf{0.17$\degree$}  & 0.044, \textbf{0.017}\\
% \midrule
% \multirow{2}{*}{Oven} & PointNet++    &  27.0$\degree$ & 0.017\\
%                       &  \nameshort     & \textbf{0.21$\degree$}  & \textbf{0.016}\\
% \midrule
% \multirow{1}{*}{Washing} & PointNet++   &  8.67$\degree$ & 0.012\\
%         Machine          &  \nameshort     & \textbf{0.12$\degree$}  & \textbf{0.006}\\
% \midrule
% \multirow{2}{*}{Laptop} & PointNet++    &  29.5$\degree$ & \textbf{0.011}\\
%                         &  \nameshort     & \textbf{0.17$\degree$}  & \textbf{0.011}\\
% \midrule
% \multirow{2}{*}{Drawer} & PointNet++   &  4.9$\degree$,5.0$\degree$,5.1$\degree$ \\
%                         &  \nameshort     & \textbf{0.13$\degree$},\textbf{0.13$\degree$},\textbf{0.13$\degree$} & -\\
%     \bottomrule
%     \end{tabular}
%     \caption{\textbf{A comparison of joint parameter predictions.}}
%     \label{tab:joint1}
% \end{table}

% \section{Real-world instance-level benchmark.}
% % - real depth result figure and comparison table [most important] 
% We have also tested our algorithm's ability  to generalize to real-world depth images on the dataset provided in \cite{michel2015pose}.  Table \ref{tab:real} shows quantitative comparison of AD accuracy. 
% \begin{table*}[h!]
%     \centering
%     \setlength\tabcolsep{4.2px}
%     \begin{tabular}{l c|c|c|c|c}
%     \toprule
%     Object               & \multicolumn{2}{c}{Sequence}  & Brachmann et al.\cite{brachmann2014learning} & Frank et al.\cite{michel2015pose} & ANCSH (Ours) \\
% \midrule
% \multirow{4}{*}{Laptop}  & \multirow{2}{*}{1}  & all     &8.9\%                 & 64.8\%                        &\textbf{94.1\%}\\
%                          &                     & parts   & 29.8\% 25.1\%                 & 65.5\% 66.9\%         &\textbf{97.5\% 94.7\%}\\
%     \cmidrule(lr){2-6}
%                          & \multirow{2}{*}{2}  & all     & 1\%                 & 65.7\%                         &\textbf{98.4\%}\\
%                          &                     & parts   & 1.1\% 63.9\%                 & 66.3\% 66.6\%         &\textbf{98.9\% 99.0\%}\\
% \midrule
% \multirow{4}{*}{Cabinet}  & \multirow{2}{*}{3}  & all    &0.5\%                 & \textbf{95.8\% }                       &90.0\%\\
%                          &                     & parts   & 86\% 46.7\% 2.6\%                & 98.2\% 97.2\% \textbf{96.1\%}        &\textbf{98.9\% 97.8\%} 91.9\%\\
%     \cmidrule(lr){2-6}
%                          & \multirow{2}{*}{4}  & all     & 49.8\%                 & \textbf{98.3\%}                         &94.5\%\\
%                          &                     & parts   & 76.8\% 85\% 74\%           & 98.3\% 98.7\% \textbf{98.7\%}       &\textbf{99.5\% 99.5\%} 94.9\%\\
% \midrule
% \multirow{4}{*}{Cupboard} & \multirow{2}{*}{5}  & all    & 90\%                 & \textbf{95.8}\%                        &93.9\%\\
%                          &                     & parts   & 91.5\% 94.3\%                & 95.9\% \textbf{95.8\%}        &\textbf{99.9\%} 93.9\%\\
%     \cmidrule(lr){2-6}
%                          & \multirow{2}{*}{6}  & all     & 71.1\%                 & 99.2\%                         &\textbf{99.9\%}\\
%                          &                     & parts   & 76.1\% 81.4\%           & 99.9\% 99.2\%        &\textbf{100\% 99.9\%}\\
% \midrule
% \multirow{4}{*}{Toy train} & \multirow{2}{*}{7}  & all     & 7.8\%                     & \textbf{98.1\%}                         &68.4\%\\
%                          &                     & parts   & 90.1\% 17.8\% 81.1\% 52.5\%  & \textbf{99.2\% 99.9\% 99.9\%} 99.1\%        &92.0\% 68.5\% 99.3\% \textbf{99.2\%}\\
%     \cmidrule(lr){2-6}
%                      & \multirow{2}{*}{8}  & all    & 5.7\%                 & \textbf{94.3\%}                      &91.1\%\\
%                          &                     & parts   & 74.8\% 20.3\% 78.2\% 51.2\%     & \textbf{100\% 100\%} 97\% \textbf{94.3\%}      &\textbf{100\% 100\% 100\%} 91.1\%\\
%     \bottomrule
%     \end{tabular}
%     \caption{\textbf{Instance-level real-world depth benchmark.} While not designed for instance-level articulated object pose estimation, our algorithm is able to achieve comparable performance compare to the state-of-the-art approach and improves the performance for challenging cases such as laptops. AD accuracy is evaluated for both the whole kinematic chain(all) and different parts(parts). }%We have greatly improved the pose estimation of laptop on the two testing sequence, on both per part and whole kinematic chain level. On other categories, we have either achieved comparable performance, or out-perform the results reported in \cite{michel2015pose}}
%     \label{tab:real}
%     \vspace{-3mm}
% \end{table*}
\section{Additional results}
 Figure \ref{fig:syn_more} shows  additional qualitative results on the synthetic dataset. More qualitative results on real-world dataset are visualized in Figure \ref{fig:real}. 

% \section{Generalization to real depth images.}
% %We also compare to the state-of-the art instance-level articulated object pose estimation approach from Michel \etal \cite{michel2015pose} on their instance-level real world depth dataset. 
% We have also tested our algorithm's ability  to generalize to real-world depth images on the dataset provided in \cite{michel2015pose}. 
% %the state-of-the art instance-level articulated object pose estimation approach from Michel \etal \cite{michel2015pose} on their instance-level real world depth dataset. 
% The dataset is designed for instance-level articulated object pose estimation, and it contains four different object instances: laptop, cupboard, 4-part toy train, and cabinet. Each has two test sequences, captured using a Kinect.
% Following the same training protocol, we train the algorithm with synthetically rendered depth images of  object instances using the URDF files provided in \cite{michel2015pose}. Then we test the pose estimation accuracy on the real world depth image.  Although our algorithm is not specifically designed for instance-level pose estimation and the network has never been trained using any real-world depth images, our algorithm achieves strong performance on par with or even better than state-of-the-art. Table \ref{tab:real} in Appendix has listed detailed performance comparison, and Figure \ref{fig:real} shows more pose estimation results on real testing data. 




% \paragraph{Occlusion visualization}
% Figure \ref{fig:occ} shows example images for each occlusion level. 
% \todo{visualization of occlusion cases (what does level1,2,3 looks like}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figure/figure7s.pdf}
    \caption{\textbf{Additional results on category-level synthetic dataset.} The first column shows the input point clouds; the second column shows our prediction and ground truth part segmentation mask; the third and fourth column show our prediction and ground truth NPCS and NAOCS, where the RGB channels encode the coordinates; the fifth column visualizes joint voting, where the arrows represent offset vectors to rotational hinge for revolute joints and the direction of joint axis for prismatic joints; the sixth column visualizes per part 3D bounding boxes, together with joint parameters. }
    \label{fig:syn_more}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.95\linewidth]{figure/figure8r.pdf}
    \caption{\textbf{Additional results on real-world instance-level depth dataset.} More qualitative results on all 4 objects from  ICCV2015 Articulated Object Challenge \cite{michel2015pose} are shown here, with toy train, cupboard, laptop, cabinet from up-pest row to lowest row in order. Only depth images are used for pose estimation, RGB images are shown here for better reference. For each object, we estimate 3D tight bounding boxes to all parts on the kinematic chain, and project the predicted bounding boxes back to the depth image. }
    \label{fig:real}
\end{figure*}



==> tex/evaluation.tex <==
\begin{table*}[t]
{
\footnotesize
\centering
\setlength\tabcolsep{4.2px}
\begin{tabular}{c|c|c|c|c|c|c|c}
\toprule
\raisebox{\dimexpr-.5\normalbaselineskip-1\cmidrulewidth-.5\aboverulesep}[0pt][0pt]{Category}                     & \raisebox{\dimexpr-.5\normalbaselineskip-1\cmidrulewidth-.5\aboverulesep}[0pt][0pt]{Method} & \multicolumn{3}{c|}{Part-based Metrics}                    & \multicolumn{1}{c|}{Joint States} & \multicolumn{2}{c}{Joint Parameters}  \\\cmidrule{3-8}
                             &        & Rotation Error $\downarrow$    &  Translation  Error  $\downarrow$      & 3D IoU $\%$ $\uparrow$         &  Error  $\downarrow$                              & Angle error  $\downarrow$          & Distance error  $\downarrow$       \\ \midrule
\multirow{2}{*}{Eye- }        &   NPCS & 4.0$\degree $, 7.7$\degree $, 7.2$\degree $      & 0.044, 0.080, 0.071          & 86.9, 40.5, 41.4    & 8.8$\degree$ ,  8.4$\degree$      & -  & -  \\
                             &  NAOCS &  4.2$\degree $, 12.1$\degree $, 13.5$\degree $ & 0.157, 0.252, 0.168       &   -                    &   13.7$\degree$, 15.1$\degree$        & -  & -                                   \\
glasses                      & \nameshort       & \textbf{3.7$\degree $, 5.1$\degree $, 3.7$\degree $}                 &  \textbf{0.035, 0.051, 0.057}              & \textbf{87.4, 43.6, 44.5}              & \bf{4.3$\degree$ , 4.5$\degree $  }          & \textbf{2.2$\degree $ ,  2.3$\degree $}	          &      	\textbf{0.019 , 0.014}                   \\  \midrule    

\multirow{3}{*}{Oven} &  NPCS     &  1.3$\degree $, 3.5$\degree $ & 0.032,	0.049 & 75.8 , 88.5  & 4.0$\degree $      & -      &     -    \\
                      &  NAOCS     &  1.7$\degree $, 4.7$\degree $               & 0.036 ,	0.090                 &   -              & 5.1$\degree$              &       -         &   -                                 \\
                       & \nameshort    &  \textbf{1.1$\degree $, 2.2$\degree $}  &\textbf{0.030},	\textbf{ 0.046}              & \textbf{75.9 , 89.0}                          & \textbf{2.1$\degree $}               & \textbf{0.8$\degree $}      &       \textbf{ 0.024 }                    \\
                              \midrule    

\multirow{2}{*}{Washing} &  NPCS     & 1.1$\degree $, 2.0$\degree $ & 0.043 ,	0.056  & 86.9 , 88.0  & 2.3 $\degree $     & -      &     - \\
                             & NAOCS & 1.1$\degree $ ,	3.3$\degree $   &   0.072 ,	0.119              &    -             &   3.1 \degree             &   -             &               -                   \\
Machine                             & \nameshort &  \textbf{1.0$\degree $ , 1.4$\degree $}  & \textbf{0.042}, \textbf{0.053}             &\textbf{ 87.0 , 88.3}                              & \textbf{1.00 $\degree $}              & \textbf{0.7$\degree $}       &          \textbf{0.008}                   \\  \midrule    

\multirow{3}{*}{Laptop} &  NPCS     &11.6$\degree $, 4.4$\degree $          & 0.098, \textbf{0.044}        & 35.7, \textbf{93.6}     & 14.4 $\degree$  & - & - \\
                        & NAOCS     &12.4$\degree $, 4.9$\degree $         & 0.110, 0.049        & -               & 15.2 $\degree$  & -   & -\\
                        & \nameshort & \textbf{6.7$\degree $, 4.3$\degree $ }       & \textbf{0.062, 0.044}     & \textbf{41.1}, 93.0     & \textbf{9.7  $\degree$}  & \textbf{0.5$\degree $}& \textbf{0.017 }      \\ \midrule 
\multirow{3}{*}{Drawer} &  NPCS     & 1.9$\degree $, 3.5$\degree $, 2.4$\degree $, 1.8$\degree $ & 0.032, 0.038, 0.024, \textbf{0.025} & 82.8, 71.2, 71.5, \textbf{79.3}   & 0.026, 0.031, 0.046 & - & -     \\
                        &  NAOCS    & 1.5$\degree $, 2.5$\degree $, 2.5$\degree $, 2.0$\degree $ & 0.044, 0.045, 0.073, 0.054 & -                        & 0.043, 0.066, 0.048 & - & -    \\
                        & \nameshort & \textbf{1.0$\degree $, 1.1$\degree $, 1.2$\degree $, 1.5$\degree $} & \textbf{0.024, 0.021, 0.021}, 0.033 & \textbf{84.0,72.1, 71.7}, 78.6   & \textbf{0.011, 0.020, 0.030} &  \textbf{0.8$\degree $, 0.8$\degree $, 0.8$\degree $} & -    \\

\bottomrule
\end{tabular}
\caption{\label{tabel:Performance comparison} \textbf{Performance comparison  on \textit{unseen} object instances.} The categories eyeglasses, oven, washing machine, and laptop contain only revolute joints and the drawer category contains three prismatic joints.}
 \vspace{-3mm}
\label{tab:syn}
}
\end{table*}

\subsection{Experimental Setup}

\paragraph{Evaluation Metrics.}
We use the following metrics to evaluate our method. %This list describes metrics for individual parts and joints.  The description that follows will describe the evaluation procecure for complete parts.
\begin{itemize}
\vspace{-2mm}\item[\Cdot]  \textbf{Part-based metrics.} 
For each part, we evaluate rotation error measured in degrees, translation error, and 3D intersection over union (IoU)~\cite{song2016deep} of the predicted amodal bounding box. 

%2) accuracy measured by percentage of pose prediction for which the error is less than $0.05$ for translation and $5\degree$ for rotation similar to \cite{shotton2013scene}. Note that to make the translation error comparable between different object instances and parts, it is measure in the normalized part coordinate space, where all part size are normalize to 1.

\vspace{-2mm}\item[\Cdot] \textbf{Joint states.}
For each revolute joint, we evaluate joint angle error in degrees. 
For each prismatic joint, we evaluate the error of relative translation amounts. 

\vspace{-2mm}\item[\Cdot]  \textbf{Joint parameters.} For each revolute joint, we evaluate the orientation error of the rotation axis in degrees, and the position error using the minimum line-to-line distance.
For each prismatic joint, we compute the orientation error of the translation axis. 
\end{itemize}

%\todo{It seems that we also need to describe how error is computed for the entire articulated object. Is it just a weighted sum of the items in the bullet list? Maybe add 1 more bullet to give a brief description.}

\mypara{Datasets.}
%\he{Whether we should merge this into Sec 4.2?}
We have evaluated our algorithm using both synthetic and real-word datasets. To generate the synthetic data, we mainly use object CAD models from \cite{wang2019shape2motion} along with drawer models from \cite{xiang2020sapien}. Following the same rendering pipeline with random camera viewpoints, we use PyBullet\cite{coumans2018} to generate on average 3000 testing images of unseen object instances for each object category that do not overlap with our training data. For the real data, we evaluated our algorithm on the dataset provided by Michel \etal \cite{michel2015pose}, which contains depth images for 4 different objects captured using the Kinect. 

\mypara{Baselines.}
There are no existing methods for category-level articulated object pose estimation. We therefore use ablated versions of our system for baseline comparison. 
\begin{itemize}
\vspace{-2mm}\item[\Cdot] \textbf{NPCS.} This algorithm predicts  part segmentation and NPCS for each part (without the joint parameters). The prediction allows the algorithm to infer part pose, amodal bounding box for each part, and joint state for revolute joint by treating each part as an independent rigid body. However, it is  not able to perform a combined optimization with the kinematic constraints.  
%\todo{Errors are reported as the weighted sum of per-part and joint errors. (?)}

\vspace{-2mm}\item[\Cdot] \textbf{NAOCS.}  This algorithm  predicts part segmentation and NAOCS representation for the whole object instance. The prediction allows the algorithm to infer part pose and joint state,  but not the amodal bounding boxes for each part since the amodal bounding boxes are not defined in the NAOCS alone. Note the part pose here is defined from the NAOCS to the camera space, different from the one we defined based upon NPCS. We measure the error in the observed object scale so that it is comparable with our method.
%\he{How does NAOCS infer the pose defined by transforming NPCS to camera space?} \xiaolong{NAOCS branch will have its own form of pose defined from NAOCS to camera space. Since the error is measured in actual object scale, we could have a fair comparison}
%\todo{In the previous sentence, what does ``it'' refer to?}
%\todo{Errors are reported as the weighted sum of per-part and joint errors. (?)}

\vspace{-2mm}\item[\Cdot] \textbf{Direct joint voting.} This algorithm directly votes for joint-associated parameters in camera space, including offset vectors and orientation for each joint from the point cloud using PointNet++  segmentation network.
%\todo{Errors are reported as the weighted sum of per-part and joint errors. (?)}
%\vspace{-2mm}\item[\Cdot] \textbf{Instance-level algorithm.} We also compare to the state-of-the art instance-level articulated object pose estimation appraoch from Michel \etal \cite{michel2015pose} on their instanceat the leaf level-level real world depth dataset. 
%\vspace{-2mm}\item[\Cdot] part nocs + joint + global scale and T  (ours final)
\end{itemize}
Our final algorithm predicts the full \nameshort representation that includes NPCS, joint parameters, and per-point global scaling and translation value that can be used together with the NPCS prediction for computing NAOCS. 


\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/figure4r.pdf}
    \caption{\textbf{Qualitative Results.} Top tow rows show test results on unseen object instances from the Shape2Motion dataset \cite{wang2019shape2motion} and SAPIEN dataset\cite{xiang2020sapien} (for only drawer category). Bottom two rows show test result on seen instances in the real-world dataset \cite{michel2015pose}. Here we visualize the predicted amodal bounding box for each parts. Color images are for visualization only. }
    \label{fig:results}
    %https://docs.google.com/drawings/d/1F8NaOgJ1scfSzYHpDyzgvS1L-cFZYJ9dTLXOvAXf4CI/edit?usp=sharing
\end{figure*}

\subsection{Experimental Results}
%, which are very good overall.
Figure~\ref{fig:results} presents some qualitative results. Tables~\ref{tab:syn} summarizes the quantitative results. 
Following paragraphs provide our analysis and discussion of the results. 

\mypara{Effect of combined optimization.}
First, we want to examine how combined optimization would influence the accuracy of articulated object pose estimation, using both predicted joint parameters and predicted part poses.    
To see this, we compare the algorithm performance between NPCS and \nameshort, where NPCS performs a per-part pose estimation and \nameshort performs a combined optimization using the full kinematic chain to constrain the result.
%
The results in Table \ref{tab:syn} show that the combined optimization of joint parameters and part pose consistently improves the predict results for almost all object categories and on almost all evaluation metrics. The improvement is particularly salient for thin object parts such as the two temples of eyeglasses (the parts that extend over the ears), where the per-part based method produces large pose errors due to limited number of visible points and shape ambiguity. 
This result demonstrates that the joint parameters predicted in the NAOCS can regularize the part poses based on kinematic chain constraints during the combined pose optimization step and improve the pose estimation accuracy. 


%The result in Table \ref{tab:syn} shows that the combine optimization of joint parameters and part pose consistently improves the algorithm's accuracy on almost all object categories and evaluation metrics. \todo{Check this}

 %The accurate joint parameters predicted in the NPCS can regularize the part poses based on kinematic chain constraints during the combined pose optimization step and  improve the pose estimation accuracy. 



%To see this, we can compare the algorithm performance between NPCS and \nameshort, where NPCS perform a per-part based pose estimation and \nameshort uses the predicted joint parameters in a combine optimization for the full kinematic chain optimization.  





\mypara{Joint parameters estimation.}
Predicting the location and the orientation of joints in camera space directly with all degrees of freedom is challenging. Our approach predicts the joint parameters in NAOCS since it provides a canonical representation where the joint axes usually have a strong orientation prior. We further use a voting-based scheme to reduce the prediction noise. Given joint axis predictions in NAOCS, we leverage the transformation between NAOCS and NPCS to compute corresponding joint parameters in NPCS. Based on the high-quality prediction of part poses, we will transform the joint parameters into the camera coordinate.
Comparing to a direct voting baseline using PointNet++, our approach significantly improves the joint axis prediction  for  unseen instances (Table \ref{tab:joint}).
%A big advantage of our algorithm is that we can accurately predict the joint parameter. 
%While most straight forward method of prediction  joint parameter is directly regress the final location and and orientation of the joint in point cloud space.
%We choose to predict joint parameter in normalized part space, 

%The result demonstrate that predicting the joint parameter in a normalize part space, and utilize voting schema can help to improve the accuracy of axis orientation prediction significantly. 



\begin{table}[h!]
    \centering
    \setlength\tabcolsep{3px}
    \begin{tabular}{c|c|c|c}
    \toprule
  Category  & Methods & Angle error & Distance error\\
\midrule
\multirow{1}{*}{Eye-} & PointNet++   &  2.9$\degree$, 15.7$\degree$ & 0.140, 0.197\\
\multirow{1}{*}{glass}         &  \nameshort     & \textbf{2.2$\degree$}, \textbf{2.3$\degree$}  & \textbf{0.019}, \textbf{0.014}\\
\midrule
\multirow{2}{*}{Oven} & PointNet++    &  27.0$\degree$ & \textbf{0.024}\\
                      &  \nameshort     & \textbf{0.8$\degree$}  & \textbf{0.024}\\
\midrule
\multirow{1}{*}{Washing} & PointNet++   &  8.7$\degree$ & 0.010\\
        Machine          &  \nameshort     & \textbf{0.7$\degree$}  & \textbf{0.008}\\
\midrule
\multirow{2}{*}{Laptop} & PointNet++    &  29.5$\degree$ & \textbf{0.007}\\
                        &  \nameshort     & \textbf{0.5$\degree$}  & 0.017\\
\midrule
\multirow{2}{*}{Drawer} & PointNet++   &  4.9$\degree$,5.0$\degree$,5.1$\degree$ & -\\
                        &  \nameshort     & \textbf{0.8$\degree$},\textbf{0.8$\degree$},\textbf{0.8$\degree$} & -\\
    \bottomrule
    \end{tabular}
    \caption{\textbf{A comparison of joint parameters estimation.} Here PointNet++ denotes the direct joint voting baseline.}
    \label{tab:joint}
    \vspace{-5mm}
\end{table}

\mypara{Generalization to real depth images.}
%We also compare to the state-of-the art instance-level articulated object pose estimation approach from Michel \etal \cite{michel2015pose} on their instance-level real world depth dataset. 
We have also tested our algorithm's ability to generalize to real-world depth images on the dataset provided in \cite{michel2015pose}. The dataset contains video sequences captured with Kinect for four different object instances. Following the same training protocol, we train the algorithm with synthetically rendered depth images of the provided object instances. Then we test the pose estimation accuracy on the real world depth images. We adopt the same evaluation metric in \cite{michel2015pose}, which uses $10 \%$ of the object part diameter as the threshold to compute Averaged Distance (AD) accuracy, and test the performance on each sequence separately. Although our algorithm is not specifically designed for instance-level pose estimation and the network has never been trained using any real-world depth images, our algorithm achieves strong performance on par with or even better than state-of-the-art. On average our algorithm achieves $96.25 \%, 92.3\%, 96.9\%, 79.8\% $ AD accuracy on the whole kinematic chain of object instance laptop, cabinet, cupboard and toy train. For detailed results on each part in all the test sequences, as well as more visualizations, please refer to the supplementary material.

% \shuran{on averge our algorithm acheives xx\% ,xx\% ,xx\%  IoU for object instance laptop, cabinet, cupboard and toy train? Detailed results and visualizations can be found in supplementary material. } %Table \ref{tab:real} in Appendix has listed detailed performance comparison, and Figure \ref{fig:real} shows more pose estimation results on real testing data.



% \shuran{not finished? } 
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \mypara{Handling prismatic joint type}
% With NPCS representation alone, the joint state for many prismatic joints like drawer is not well defined. 
% \todo{@He or @Eric, need help on this. or do we need this?}
%Table \ref{tab:real} show the performance comparison. 
%compare to the state-of-the-art, and outperforms in some of the challenging cases (\eg on laptop).
% \begin{table*}[h!]
%     \centering
%     \setlength\tabcolsep{4.2px}
%     \begin{tabular}{l c|c|c|c|c}
%     \toprule
%     Object               & \multicolumn{2}{c}{Sequence}  & Brachmann et al.\cite{brachmann2014learning} & Frank et al.\cite{michel2015pose} & A-NCSH (Ours) \\
% \midrule
% \multirow{4}{*}{Laptop}  & \multirow{2}{*}{1}  & all     &8.9\%                 & 64.8\%                        &\textbf{94.1\%}\\
%                          &                     & parts   & 29.8\% 25.1\%                 & 65.5\% 66.9\%         &\textbf{97.5\% 94.7\%}\\
%     \cmidrule(lr){2-6}
%                          & \multirow{2}{*}{2}  & all     & 1\%                 & 65.7\%                         &\textbf{98.4\%}\\
%                          &                     & parts   & 1.1\% 63.9\%                 & 66.3\% 66.6\%         &\textbf{98.9\% 99.0\%}\\
% \midrule
% \multirow{4}{*}{Cabinet}  & \multirow{2}{*}{3}  & all    &0.5\%                 & \textbf{95.8\% }                       &90.0\%\\
%                          &                     & parts   & 86\% 46.7\% 2.6\%                & 98.2\% 97.2\% \textbf{96.1\%}        &\textbf{98.9\% 97.8\%} 91.9\%\\
%     \cmidrule(lr){2-6}
%                          & \multirow{2}{*}{4}  & all     & 49.8\%                 & \textbf{98.3\%}                         &94.5\%\\
%                          &                     & parts   & 76.8\% 85\% 74\%           & 98.3\% 98.7\% \textbf{98.7\%}       &\textbf{99.5\% 99.5\%} 94.9\%\\
% \midrule
% \multirow{4}{*}{Cupboard} & \multirow{2}{*}{5}  & all    & 90\%                 & 95.8\%                        &93.9\%\\
%                          &                     & parts   & 91.5\% 94.3\%                & 95.9\% \textbf{95.8\%}        &\textbf{99.9\%} 93.9\%\\
%     \cmidrule(lr){2-6}
%                          & \multirow{2}{*}{6}  & all     & 71.1\%                 & 99.2\%                         &\textbf{99.9\%}\\
%                          &                     & parts   & 76.1\% 81.4\%           & 99.9\% 99.2\%        &\textbf{100\% 99.9\%}\\
% \midrule
% \multirow{4}{*}{Toy train} & \multirow{2}{*}{7}  & all     & 7.8\%                     & \textbf{98.1\%}                         &68.4\%\\
%                          &                     & parts   & 90.1\% 17.8\% 81.1\% 52.5\%  & \textbf{99.2\% 99.9\% 99.9\%} 99.1\%        &92.0\% 68.5\% 99.3\% \textbf{99.2\%}\\
%     \cmidrule(lr){2-6}
%                      & \multirow{2}{*}{8}  & all    & 5.7\%                 & \textbf{94.3\%}                      &91.1\%\\
%                          &                     & parts   & 74.8\% 20.3\% 78.2\% 51.2\%     & \textbf{100\% 100\%} 97\% \textbf{94.3\%}      &\textbf{100\% 100\% 100\%} 91.1\%\\
%     \bottomrule
%     \end{tabular}
%     \caption{\textbf{Instance-level real-world depth benchmark.} While not designed for instance-level articulated object pose estimation, our algorithm is able to achieve comparable performance compare to the state-of-the-art approach and improves the performance for challenging cases such as laptops. \todo{should we include it in appendix?} }%We have greatly improved the pose estimation of laptop on the two testing sequence, on both per part and whole kinematic chain level. On other categories, we have either achieved comparable performance, or out-perform the results reported in \cite{michel2015pose}}
%     \label{tab:real}
%     \vspace{-3mm}
% \end{table*}

